Molecular gas in super spiral galaxies

At the highest stellar masses (log(\mstar) $\gtrsim$ 11.5 \msun), only a small fraction of galaxies are disk-like and actively star-forming objects. These so-called `super spirals' are ideal objects to better understand how galaxy evolution proceeds and to extend our knowledge about the relation between stars and gas to a higher stellar mass regime. We present new CO(1-0) data for a sample of 46 super spirals and for 18 slightly lower-mass (log(\mstar) $>$ 11.0 \msun ) galaxies with broad HI lines -- HI fast-rotators (HI-FRs). We analyze their molecular gas mass, derived from CO, in relation to their star formation rate (SFR) and stellar mass, and compare the results to values and scaling relations derived from lower-mass galaxies. We confirm that super spirals follow the same star-forming main sequence (SFMS) as lower-mass galaxies. We find that they possess abundant molecular gas, which lies above the extrapolation of the scaling relation with stellar mass derived from lower-mass galaxies, but within the relation between \mmol/\mstar and the distance to the SFMS. The molecular gas depletion time, \taudep = \mmol/SFR, is higher than for lower-mass galaxies on the SFMS (\taudep = 9.30 $\pm$ 0.03, compared to \taudep = 9.00 $\pm$ 0.02 for the comparison sample) and seems to continue an increasing trend with stellar mass. HI-FR galaxies have an atomic-to-molecular gas mass ratio that is in agreement with that of lower-mass galaxies, indicating that the conversion from the atomic to molecular gas proceeds in a similar way. We conclude that the availability of molecular gas is a crucial factor to enable star formation to continue and that, if gas is present, quenching is not a necessary destiny for high-mass galaxies. The difference in gas depletion time suggests that the properties of the molecular gas at high stellar masses are less favorable for star formation.

==> Table1.tex <==
2MFGC12344 &   0.88 &   1.57 $\pm$   0.13 & 0 &   1018 \\ 
OGC~139 &   1.67 & $<$   0.60 & 1 &    700 \\ 
OGC~217 &   1.67 &   1.39 $\pm$   0.14 & 0 &    347 \\ 
OGC~290 &   1.46 &   1.02 $\pm$   0.13 & 0 &    403 \\ 
OGC~345 &   1.25 &   1.36 $\pm$   0.14 & 0 &    601 \\ 
OGC~454 &   1.71 &   0.96 $\pm$   0.16 & 0 &    454 \\ 
OGC~543 &   1.65 &   1.91 $\pm$   0.17 & 0 &    497 \\ 
OGC~586 &   1.53 &   2.04 $\pm$   0.20 & 0 &    853 \\ 
OGC~595 &   1.35 &   0.69 $\pm$   0.13 & 0 &    427 \\ 
OGC~789 &   1.70 &   1.49 $\pm$   0.11 & 0 &    197 \\ 
OGC~800 &   1.25 &   1.61 $\pm$   0.15 & 0 &    651 \\ 
OGC~830 &   1.12 &   0.62 $\pm$   0.12 & 0 &    610 \\ 
OGC~926 &   1.67 &   2.29 $\pm$   0.19 & 0 &    631 \\ 
OGC~928 &   2.54 & $<$   0.91 & 1 &    700 \\ 
OGC~968 &   1.10 &   1.21 $\pm$   0.13 & 0 &    673 \\ 
OGC~1250 &   1.15 &   1.19 $\pm$   0.12 & 0 &    555 \\ 
OGC~1273 &   1.29 &   0.57 $\pm$   0.15 & 2 &    679 \\ 
OGC~1304 &   0.92 &   0.92 $\pm$   0.11 & 0 &    693 \\ 
OGC~1379 &   1.57 &   0.61 $\pm$   0.20 & 2 &    792 \\ 
OGC~1457 &   1.07 &   0.74 $\pm$   0.10 & 0 &    442 \\ 
OGC~1464 &   1.13 &   1.11 $\pm$   0.12 & 0 &    595 \\ 
OGC~1501 &   1.49 &   1.65 $\pm$   0.16 & 0 &    538 \\ 
OGC~1546 &   1.30 &   0.67 $\pm$   0.12 & 0 &    430 \\ 
OGC~1559 &   1.05 &   2.03 $\pm$   0.12 & 0 &    629 \\ 
J00493937+1341067 &   1.69 &   2.46 $\pm$   0.20 & 0 &    727 \\ 
J01593759+1231120 &   2.13 &   2.42 $\pm$   0.21 & 0 &    481 \\ 
J03091553+0025080 &   1.64 &   1.43 $\pm$   0.17 & 0 &    534 \\ 
J03502457+0058530 &   1.77 &   1.50 $\pm$   0.21 & 0 &    653 \\ 
J07521780+1935423 &   1.29 &   0.48 $\pm$   0.10 & 0 &    277 \\ 
J08045271+2120504 &   0.95 &   0.49 $\pm$   0.11 & 2 &    697 \\ 
J08055992+2606027 &   1.28 &   0.81 $\pm$   0.16 & 0 &    805 \\ 
J08185186+1013117 &   1.62 &   2.04 $\pm$   0.20 & 0 &    753 \\ 
J08211000+0748139 &   1.29 & $<$   0.46 & 1 &    700 \\ 
J08293057+0812383 &   1.25 &   0.70 $\pm$   0.13 & 0 &    560 \\ 
J09044020+1725124 &   1.56 &   2.20 $\pm$   0.18 & 0 &    604 \\ 
J09072322+0948348 &   1.52 &   1.54 $\pm$   0.20 & 0 &    904 \\ 
J09142624+1024093 &   1.31 &   1.55 $\pm$   0.16 & 0 &    723 \\ 
J09193819+3336120 &   2.01 &   1.55 $\pm$   0.22 & 0 &    589 \\ 
J09354887+0937188 &   1.26 &   1.41 $\pm$   0.14 & 0 &    597 \\ 
J09381483+0200236 &   1.46 &   0.81 $\pm$   0.14 & 0 &    416 \\ 
J09405816+1904371 &   1.50 &   2.02 $\pm$   0.21 & 0 &    977 \\ 
J09473320+1005093 &   1.01 &   0.49 $\pm$   0.09 & 0 &    388 \\ 
J10005570+3140007 &   1.88 &   0.73 $\pm$   0.10 & 0 &    151 \\ 
J10222648+0911396 &   1.31 &   1.57 $\pm$   0.15 & 0 &    594 \\ 
J10335255+0044033 &   0.94 &   0.34 $\pm$   0.11 & 2 &    661 \\ 
J10340239+3452104 &   3.19 &  17.21 $\pm$   0.25 & 0 &    308 \\ 
J10375221+3125004 &   1.59 &   0.56 $\pm$   0.16 & 2 &    489 \\ 
J10500776+1132290 &   1.23 &   1.11 $\pm$   0.13 & 0 &    543 \\ 
J10500425+1205195 &   2.81 &   1.81 $\pm$   0.16 & 0 &    171 \\ 
J10523297+1036205 &   2.21 &   2.28 $\pm$   0.27 & 0 &    748 \\ 
J10542879+2049141 &   1.19 &   1.10 $\pm$   0.14 & 0 &    697 \\ 
J11052843+0736413 &   1.32 &   1.19 $\pm$   0.19 & 0 &    981 \\ 
J11302884+1301197 &   1.39 &   0.62 $\pm$   0.18 & 2 &    814 \\ 
J11341760+1751336 &   1.22 &   0.91 $\pm$   0.16 & 0 &    835 \\ 
J11444504+1111056 &   1.43 & $<$   0.51 & 1 &    700 \\ 
J12063088+2221045 &   1.99 &   2.96 $\pm$   0.19 & 0 &    436 \\ 
J12284130+0725421 &   1.43 &   1.31 $\pm$   0.17 & 0 &    710 \\ 
J12393314+1058037 &   1.96 &   2.34 $\pm$   0.19 & 0 &    444 \\ 
J12533769+2126177 &   1.02 & $<$   0.36 & 1 &    700 \\ 
J13003624+1347055 &   1.26 &   0.78 $\pm$   0.15 & 0 &    748 \\ 
J13390599+1627261 &   1.93 & $<$   0.69 & 1 &    700 \\ 
J13413717+0848096 &   1.46 &   2.11 $\pm$   0.19 & 0 &    866 \\ 
J13473338+1217245 &   1.24 &   3.54 $\pm$   0.15 & 0 &    725 \\ 
J14014270+0119379 &   1.40 &   0.93 $\pm$   0.12 & 0 &    363 \\ 
J14131920+3649184 &   1.69 &   1.23 $\pm$   0.20 & 0 &    711 \\ 
J14190190+2809409 &   1.42 &   1.36 $\pm$   0.14 & 0 &    503 \\ 
J14322461+0050419 &   1.52 &   0.84 $\pm$   0.16 & 0 &    572 \\ 
J14394590+2018469 &   1.32 &   1.11 $\pm$   0.17 & 0 &    838 \\ 
J15051087+0503026 &   2.24 &   4.69 $\pm$   0.25 & 0 &    608 \\ 
J15590130+1610517 &   1.76 &   2.07 $\pm$   0.19 & 0 &    564 \\ 
J16045551+2809563 &   2.18 &   3.78 $\pm$   0.23 & 0 &    540 \\ 
J16373623+2022167 &   1.25 &   1.56 $\pm$   0.15 & 0 &    668 \\ 
J21020534-0647558 &   2.15 &   1.28 $\pm$   0.23 & 0 &    559 \\ 
J23463606+1356475 &   1.30 &   2.13 $\pm$   0.18 & 0 &    978 \\ 
IC2218 &   1.68 &   1.48 $\pm$   0.20 & 0 &    659 \\ 
NGC2620 &   3.01 &   1.89 $\pm$   0.30 & 0 &    472 \\ 
NGC2713 &   3.44 &   4.09 $\pm$   0.40 & 0 &    631 \\ 
IC2446 &   3.78 &   7.37 $\pm$   0.46 & 0 &    738 \\ 
IC536 &   2.01 &   1.70 $\pm$   0.27 & 0 &    876 \\ 
UGC05830 &   2.23 &   6.82 $\pm$   0.26 & 0 &    621 \\ 
UGC06066 &   1.04 &   0.45 $\pm$   0.13 & 2 &    738 \\ 
UGC08179 &   2.24 &   9.90 $\pm$   0.29 & 0 &    830 \\ 
IC881 &   1.75 & $<$   0.62 & 1 &    700 \\ 
UGC08902 &   2.94 &   8.08 $\pm$   0.35 & 0 &    708 \\ 
NGC5417 &   2.51 & $<$   0.91 & 1 &    700 \\ 
NGC5440 &   2.65 &   3.14 $\pm$   0.33 & 0 &    718 \\ 
UGC09195 &   1.42 &   2.06 $\pm$   0.17 & 0 &    725 \\ 
NGC5635 &   2.30 &   2.13 $\pm$   0.26 & 0 &    622 \\ 
NGC5790 &   1.96 &   2.13 $\pm$   0.24 & 0 &    703 \\ 
UGC09757 &   3.61 &   5.71 $\pm$   0.42 & 0 &    683 \\ 
UGC09795 &   3.42 &   4.99 $\pm$   0.42 & 0 &    756 \\ 
UGC12591 &   1.95 &   2.65 $\pm$   0.29 & 0 &   1091 \\ 


==> Table2.tex <==
2MFGC12344 &  0.141 &    665 &  10.58 $\pm$   0.15 &   1.17 \\ 
OGC~139 &  0.247 &   1244 & $<$  10.66  &   1.15 \\ 
OGC~217 &  0.249 &   1254 &  10.99 $\pm$   0.16 &   1.05 \\ 
OGC~290 &  0.296 &   1528 &  11.01 $\pm$   0.17 &   1.05 \\ 
OGC~345 &  0.222 &   1104 &  10.89 $\pm$   0.16 &   1.08 \\ 
OGC~454 &  0.259 &   1310 &  10.86 $\pm$   0.18 &   1.03 \\ 
OGC~543 &  0.109 &    505 &  10.53 $\pm$   0.15 &   1.46 \\ 
OGC~586 &  0.167 &    801 &  10.85 $\pm$   0.15 &   1.18 \\ 
OGC~595 &  0.223 &   1105 &  10.60 $\pm$   0.19 &   1.09 \\ 
OGC~789 &  0.157 &    748 &  10.62 $\pm$   0.14 &   1.08 \\ 
OGC~800 &  0.144 &    681 &  10.60 $\pm$   0.15 &   1.14 \\ 
OGC~830 &  0.158 &    753 &  10.26 $\pm$   0.19 &   1.14 \\ 
OGC~926 &  0.161 &    770 &  10.86 $\pm$   0.15 &   1.16 \\ 
OGC~928 &  0.273 &   1391 & $<$  10.88  &   1.03 \\ 
OGC~968 &  0.219 &   1086 &  10.81 $\pm$   0.16 &   1.04 \\ 
OGC~1250 &  0.166 &    797 &  10.60 $\pm$   0.16 &   1.16 \\ 
OGC~1273 &  0.231 &   1152 &  10.53 $\pm$   0.22 &   1.04 \\ 
OGC~1304 &  0.164 &    789 &  10.57 $\pm$   0.16 &   1.43 \\ 
OGC~1379 &  0.179 &    869 &  10.35 $\pm$   0.23 &   1.07 \\ 
OGC~1457 &  0.239 &   1198 &  10.67 $\pm$   0.17 &   1.04 \\ 
OGC~1464 &  0.298 &   1543 &  11.09 $\pm$   0.16 &   1.13 \\ 
OGC~1501 &  0.172 &    830 &  10.74 $\pm$   0.15 &   1.07 \\ 
OGC~1546 &  0.137 &    647 &  10.17 $\pm$   0.19 &   1.13 \\ 
OGC~1559 &  0.089 &    407 &  10.44 $\pm$   0.14 &   1.69 \\ 
J00493937+1341067 &  0.133 &    626 &  10.70 $\pm$   0.15 &   1.10 \\ 
J01593759+1231120 &  0.164 &    786 &  10.85 $\pm$   0.15 &   1.04 \\ 
J03091553+0025080 &  0.108 &    500 &  10.28 $\pm$   0.16 &   1.10 \\ 
J03502457+0058530 &  0.165 &    791 &  10.66 $\pm$   0.17 &   1.05 \\ 
J07521780+1935423 &  0.117 &    546 &   9.89 $\pm$   0.19 &   1.13 \\ 
J08045271+2120504 &  0.125 &    583 &   9.94 $\pm$   0.20 &   1.11 \\ 
J08055992+2606027 &  0.137 &    644 &  10.23 $\pm$   0.19 &   1.07 \\ 
J08185186+1013117 &  0.082 &    371 &  10.24 $\pm$   0.15 &   1.25 \\ 
J08211000+0748139 &  0.198 &    970 & $<$  10.31  &   1.06 \\ 
J08293057+0812383 &  0.130 &    608 &  10.11 $\pm$   0.19 &   1.06 \\ 
J09044020+1725124 &  0.093 &    424 &  10.38 $\pm$   0.15 &   1.25 \\ 
J09072322+0948348 &  0.180 &    869 &  10.75 $\pm$   0.17 &   1.06 \\ 
J09142624+1024093 &  0.176 &    851 &  10.74 $\pm$   0.16 &   1.09 \\ 
J09193819+3336120 &  0.165 &    794 &  10.69 $\pm$   0.17 &   1.09 \\ 
J09354887+0937188 &  0.133 &    627 &  10.47 $\pm$   0.15 &   1.14 \\ 
J09381483+0200236 &  0.175 &    843 &  10.47 $\pm$   0.18 &   1.13 \\ 
J09405816+1904371 &  0.159 &    762 &  10.76 $\pm$   0.16 &   1.06 \\ 
J09473320+1005093 &  0.140 &    659 &  10.05 $\pm$   0.19 &   1.12 \\ 
J10005570+3140007 &  0.195 &    953 &  10.48 $\pm$   0.17 &   1.03 \\ 
J10222648+0911396 &  0.091 &    418 &  10.23 $\pm$   0.15 &   1.27 \\ 
J10335255+0044033 &  0.132 &    618 &   9.83 $\pm$   0.24 &   1.12 \\ 
J10340239+3452104 &  0.071 &    320 &  10.99 $\pm$   0.12 &   1.11 \\ 
J10375221+3125004 &  0.160 &    765 &  10.23 $\pm$   0.22 &   1.13 \\ 
J10500776+1132290 &  0.133 &    628 &  10.36 $\pm$   0.16 &   1.11 \\ 
J10500425+1205195 &  0.135 &    638 &  10.60 $\pm$   0.15 &   1.15 \\ 
J10523297+1036205 &  0.088 &    401 &  10.60 $\pm$   0.16 &   2.20 \\ 
J10542879+2049141 &  0.191 &    929 &  10.65 $\pm$   0.17 &   1.04 \\ 
J11052843+0736413 &  0.152 &    725 &  10.55 $\pm$   0.18 &   1.23 \\ 
J11302884+1301197 &  0.135 &    637 &  10.11 $\pm$   0.22 &   1.09 \\ 
J11341760+1751336 &  0.180 &    874 &  10.53 $\pm$   0.18 &   1.09 \\ 
J11444504+1111056 &  0.153 &    730 & $<$  10.13  &   1.06 \\ 
J12063088+2221045 &  0.106 &    491 &  10.60 $\pm$   0.14 &   1.15 \\ 
J12284130+0725421 &  0.163 &    781 &  10.59 $\pm$   0.17 &   1.06 \\ 
J12393314+1058037 &  0.075 &    338 &  10.16 $\pm$   0.15 &   1.09 \\ 
J12533769+2126177 &  0.127 &    597 & $<$   9.80  &   1.03 \\ 
J13003624+1347055 &  0.142 &    672 &  10.25 $\pm$   0.19 &   1.09 \\ 
J13390599+1627261 &  0.173 &    832 & $<$  10.36  &   1.04 \\ 
J13413717+0848096 &  0.079 &    356 &  10.26 $\pm$   0.15 &   1.39 \\ 
J13473338+1217245 &  0.122 &    568 &  10.79 $\pm$   0.13 &   1.13 \\ 
J14014270+0119379 &  0.139 &    656 &  10.31 $\pm$   0.17 &   1.09 \\ 
J14131920+3649184 &  0.172 &    828 &  10.61 $\pm$   0.18 &   1.06 \\ 
J14190190+2809409 &  0.138 &    651 &  10.47 $\pm$   0.16 &   1.09 \\ 
J14322461+0050419 &  0.124 &    582 &  10.22 $\pm$   0.19 &   1.24 \\ 
J14394590+2018469 &  0.119 &    554 &  10.26 $\pm$   0.18 &   1.13 \\ 
J15051087+0503026 &  0.074 &    333 &  10.56 $\pm$   0.14 &   1.42 \\ 
J15590130+1610517 &  0.139 &    655 &  10.67 $\pm$   0.15 &   1.13 \\ 
J16045551+2809563 &  0.077 &    349 &  10.50 $\pm$   0.14 &   1.40 \\ 
J16373623+2022167 &  0.118 &    549 &  10.39 $\pm$   0.15 &   1.10 \\ 
J21020534-0647558 &  0.127 &    597 &  10.37 $\pm$   0.18 &   1.08 \\ 
J23463606+1356475 &  0.117 &    542 &  10.54 $\pm$   0.15 &   1.16 \\ 
IC2218 &  0.043 &    191 &   9.59 $\pm$   0.17 &   1.40 \\ 
NGC2620 &  0.026 &    114 &   9.53 $\pm$   0.18 &   2.66 \\ 
NGC2713 &  0.013 &     57 &   9.63 $\pm$   0.15 &   6.13 \\ 
IC2446 &  0.026 &    116 &  10.09 $\pm$   0.14 &   2.42 \\ 
IC536 &  0.027 &    119 &   9.31 $\pm$   0.18 &   1.63 \\ 
UGC05830 &  0.044 &    195 &  10.28 $\pm$   0.13 &   1.45 \\ 
UGC06066 &  0.039 &    174 &   9.11 $\pm$   0.22 &   1.83 \\ 
UGC08179 &  0.052 &    230 &  10.65 $\pm$   0.13 &   1.67 \\ 
IC881 &  0.023 &    102 & $<$   8.84  &   2.08 \\ 
UGC08902 &  0.026 &    112 &  10.07 $\pm$   0.13 &   2.25 \\ 
NGC5417 &  0.016 &     71 & $<$   8.87  &   3.12 \\ 
NGC5440 &  0.012 &     53 &   9.47 $\pm$   0.16 &   6.26 \\ 
UGC09195 &  0.050 &    222 &  10.03 $\pm$   0.15 &   2.06 \\ 
NGC5635 &  0.014 &     62 &   9.32 $\pm$   0.16 &   4.84 \\ 
NGC5790 &  0.037 &    162 &   9.78 $\pm$   0.16 &   2.07 \\ 
UGC09757 &  0.040 &    177 &  10.17 $\pm$   0.15 &   1.61 \\ 
UGC09795 &  0.044 &    196 &  10.21 $\pm$   0.15 &   1.67 \\ 
UGC12591 &  0.023 &    101 &   9.55 $\pm$   0.16 &   2.39 \\ 


==> Table4.tex <==
2MFGC12344 &   3.14 $\pm$   0.10 &   4.56 $\pm$   0.05 &   1.81 $\pm$   0.09 &   2.75 $\pm$   0.03 &   3.24 $\pm$   0.60 &   4.17 $\pm$   0.19&   5.52 $\pm$   0.99 &   5.54 $\pm$   0.89 & SS\\ 
OGC~139 &   0.90 $\pm$   0.04 &   1.68 $\pm$   0.02 &   0.57 $\pm$   0.04 &   1.27 $\pm$   0.02 &   1.47 $\pm$   0.12 &   2.65 $\pm$   0.10&   2.20 $\pm$   0.80 &   2.65 $\pm$   0.59 & SS\\ 
OGC~217 &   0.72 $\pm$   0.03 &   1.23 $\pm$   0.02 &   0.51 $\pm$   0.04 &   1.10 $\pm$   0.02 &   4.23 $\pm$   0.23 &   5.26 $\pm$   0.16&  14.19 $\pm$   1.20 &   6.67 $\pm$   0.69 & SS\\ 
OGC~290 &   0.59 $\pm$   0.03 &   1.20 $\pm$   0.02 &   0.41 $\pm$   0.03 &   1.07 $\pm$   0.01 &   2.28 $\pm$   0.20 &   3.04 $\pm$   0.15&   6.77 $\pm$   1.13 &   3.43 $\pm$   0.57 & SS\\ 
OGC~345 &   1.05 $\pm$   0.04 &   1.83 $\pm$   0.02 &   0.67 $\pm$   0.05 &   1.39 $\pm$   0.03 &   2.06 $\pm$   0.31 &   3.36 $\pm$   0.28&   3.44 $\pm$   1.98 &   3.87 $\pm$   1.35 & SS\\ 
OGC~454 &   0.64 $\pm$   0.03 &   1.17 $\pm$   0.02 &   0.46 $\pm$   0.03 &   1.01 $\pm$   0.02 &   2.94 $\pm$   0.22 &   4.05 $\pm$   0.16&   4.48 $\pm$   1.36 &   3.65 $\pm$   0.78 & SS\\ 
OGC~543 &   4.14 $\pm$   0.14 &   5.94 $\pm$   0.07 &   2.62 $\pm$   0.11 &   3.84 $\pm$   0.06 &   8.08 $\pm$   0.64 &   9.00 $\pm$   0.32&  10.07 $\pm$   1.82 &  10.46 $\pm$   1.54 & SS\\ 
OGC~586 &   1.68 $\pm$   0.06 &   2.73 $\pm$   0.03 &   1.11 $\pm$   0.06 &   1.89 $\pm$   0.03 &   4.42 $\pm$   0.23 &   6.15 $\pm$   0.16&   8.15 $\pm$   1.02 &   5.31 $\pm$   0.53 & SS\\ 
OGC~595 &   0.68 $\pm$   0.03 &   1.24 $\pm$   0.02 &   0.44 $\pm$   0.04 &   0.91 $\pm$   0.03 &   1.66 $\pm$   0.23 &   2.20 $\pm$   0.17&  -2.14 $\pm$   0.00 &   1.24 $\pm$   0.83 & SS\\ 
OGC~789 &   1.81 $\pm$   0.06 &   2.69 $\pm$   0.03 &   1.13 $\pm$   0.06 &   1.87 $\pm$   0.04 &   3.72 $\pm$   0.29 &   5.65 $\pm$   0.25&   5.56 $\pm$   1.69 &   5.27 $\pm$   1.24 & SS\\ 
OGC~800 &   2.30 $\pm$   0.08 &   3.41 $\pm$   0.04 &   1.36 $\pm$   0.07 &   2.21 $\pm$   0.04 &   2.89 $\pm$   0.28 &   4.34 $\pm$   0.24&   4.65 $\pm$   1.73 &   3.76 $\pm$   1.16 & SS\\ 
OGC~830 &   2.00 $\pm$   0.07 &   3.07 $\pm$   0.04 &   1.14 $\pm$   0.06 &   1.96 $\pm$   0.02 &   2.40 $\pm$   0.16 &   3.54 $\pm$   0.13&   4.99 $\pm$   0.93 &   3.88 $\pm$   0.64 & SS\\ 
OGC~926 &   1.91 $\pm$   0.07 &   3.04 $\pm$   0.03 &   1.35 $\pm$   0.06 &   2.21 $\pm$   0.03 &   6.75 $\pm$   0.35 &   8.37 $\pm$   0.22&  13.20 $\pm$   1.61 &   7.49 $\pm$   0.82 & SS\\ 
OGC~928 &   0.59 $\pm$   0.03 &   1.21 $\pm$   0.02 &   0.39 $\pm$   0.04 &   0.94 $\pm$   0.03 &   1.53 $\pm$   0.14 &   2.14 $\pm$   0.10&   1.89 $\pm$   0.90 &   1.86 $\pm$   0.50 & SS\\ 
OGC~968 &   0.86 $\pm$   0.04 &   1.51 $\pm$   0.02 &   0.63 $\pm$   0.04 &   1.26 $\pm$   0.02 &   3.64 $\pm$   0.26 &   4.78 $\pm$   0.21&  15.59 $\pm$   1.58 &  11.02 $\pm$   1.01 & SS\\ 
OGC~1250 &   1.19 $\pm$   0.04 &   1.87 $\pm$   0.02 &   0.75 $\pm$   0.04 &   1.36 $\pm$   0.02 &   1.88 $\pm$   0.19 &   2.75 $\pm$   0.16&  -2.75 $\pm$   0.00 &   1.56 $\pm$   0.81 & SS\\ 
OGC~1273 &   0.62 $\pm$   0.03 &   1.11 $\pm$   0.02 &   0.41 $\pm$   0.04 &   0.89 $\pm$   0.03 &   1.23 $\pm$   0.27 &   1.95 $\pm$   0.24&  -2.26 $\pm$   0.00 &   1.72 $\pm$   1.13 & SS\\ 
OGC~1304 &   1.70 $\pm$   0.06 &   2.57 $\pm$   0.04 &   1.04 $\pm$   0.06 &   1.80 $\pm$   0.02 &   2.61 $\pm$   0.14 &   3.59 $\pm$   0.11&   4.80 $\pm$   0.98 &   3.42 $\pm$   0.53 & SS\\ 
OGC~1379 &   1.16 $\pm$   0.04 &   1.90 $\pm$   0.02 &   0.74 $\pm$   0.05 &   1.36 $\pm$   0.04 &   2.64 $\pm$   0.26 &   3.05 $\pm$   0.21&   7.13 $\pm$   1.69 &   4.85 $\pm$   1.05 & SS\\ 
OGC~1457 &   0.54 $\pm$   0.03 &   0.94 $\pm$   0.02 &   0.38 $\pm$   0.04 &   0.78 $\pm$   0.03 &   3.01 $\pm$   0.31 &   3.83 $\pm$   0.26&  17.04 $\pm$   2.01 &   4.41 $\pm$   1.28 & SS\\ 
OGC~1464 &   0.46 $\pm$   0.02 &   0.89 $\pm$   0.01 &   0.34 $\pm$   0.02 &   0.78 $\pm$   0.01 &   2.66 $\pm$   0.21 &   3.56 $\pm$   0.14&   4.12 $\pm$   1.14 &   3.04 $\pm$   0.58 & SS\\ 
OGC~1501 &   2.66 $\pm$   0.08 &   3.67 $\pm$   0.04 &   3.09 $\pm$   0.12 &   4.05 $\pm$   0.05 &   9.03 $\pm$   0.40 &  10.94 $\pm$   0.25&  33.73 $\pm$   2.41 &  24.08 $\pm$   1.65 & SS\\ 
OGC~1546 &   2.35 $\pm$   0.08 &   3.54 $\pm$   0.04 &   1.36 $\pm$   0.07 &   2.27 $\pm$   0.04 &   1.88 $\pm$   0.16 &   2.41 $\pm$   0.11&   2.54 $\pm$   0.87 &   1.71 $\pm$   0.44 & SS\\ 
OGC~1559 &   6.87 $\pm$   0.21 &   9.39 $\pm$   0.10 &   4.00 $\pm$   0.15 &   5.56 $\pm$   0.06 &   7.10 $\pm$   0.41 &   9.99 $\pm$   0.32&  10.34 $\pm$   1.63 &   8.92 $\pm$   1.53 & SS\\ 
J00493937+1341067 &   2.56 $\pm$   0.07 &   3.15 $\pm$   0.04 &   3.28 $\pm$   0.12 &   4.19 $\pm$   0.05 &  16.86 $\pm$   0.49 &  15.99 $\pm$   0.32&  48.79 $\pm$   2.82 &  44.93 $\pm$   2.08 & SS\\ 
J01593759+1231120 &   1.48 $\pm$   0.05 &   2.12 $\pm$   0.03 &   0.99 $\pm$   0.05 &   1.64 $\pm$   0.02 &   5.15 $\pm$   0.26 &   6.86 $\pm$   0.17&   9.12 $\pm$   1.28 &   6.57 $\pm$   0.79 & SS\\ 
J03091553+0025080 &   5.99 $\pm$   0.16 &   6.99 $\pm$   0.08 &   7.23 $\pm$   0.24 &   8.65 $\pm$   0.09 &  17.66 $\pm$   0.76 &  19.74 $\pm$   0.33&  33.75 $\pm$   2.18 &  38.38 $\pm$   1.69 & SS\\ 
J03502457+0058530 &   1.72 $\pm$   0.05 &   2.31 $\pm$   0.03 &   1.86 $\pm$   0.08 &   2.49 $\pm$   0.04 &   6.68 $\pm$   0.35 &   7.48 $\pm$   0.30&  42.17 $\pm$   2.23 &  31.59 $\pm$   1.55 & SS\\ 
J07521780+1935423 &   8.31 $\pm$   0.22 &   9.68 $\pm$   0.10 &  11.87 $\pm$   0.39 &  14.74 $\pm$   0.16 &  37.42 $\pm$   0.97 &  40.03 $\pm$   0.52& 150.21 $\pm$   4.49 & 139.62 $\pm$   2.52 & SS\\ 
J08045271+2120504 &   4.19 $\pm$   0.12 &   5.34 $\pm$   0.06 &   5.48 $\pm$   0.19 &   6.69 $\pm$   0.08 &  11.80 $\pm$   0.45 &  15.18 $\pm$   0.30&  37.53 $\pm$   2.09 &  29.58 $\pm$   1.51 & SS\\ 
J08055992+2606027 &   3.97 $\pm$   0.11 &   4.90 $\pm$   0.05 &   4.52 $\pm$   0.16 &   5.70 $\pm$   0.07 &  10.43 $\pm$   0.40 &  11.96 $\pm$   0.28&  22.26 $\pm$   2.45 &  25.05 $\pm$   1.90 & SS\\ 
J08185186+1013117 &   4.35 $\pm$   0.13 &   5.61 $\pm$   0.06 &   2.60 $\pm$   0.10 &   3.53 $\pm$   0.04 &   6.37 $\pm$   0.35 &   8.69 $\pm$   0.30&   7.25 $\pm$   1.88 &   6.14 $\pm$   1.45 & SS\\ 
J08211000+0748139 &   1.38 $\pm$   0.04 &   1.57 $\pm$   0.02 &   1.84 $\pm$   0.05 &   2.20 $\pm$   0.03 &   6.59 $\pm$   0.36 &   6.39 $\pm$   0.26&  17.09 $\pm$   1.77 &  12.25 $\pm$   1.01 & SS\\ 
J08293057+0812383 &   4.80 $\pm$   0.13 &   5.59 $\pm$   0.06 &   6.60 $\pm$   0.21 &   7.72 $\pm$   0.09 &  18.92 $\pm$   0.59 &  21.71 $\pm$   0.37&  52.64 $\pm$   2.63 &  51.12 $\pm$   1.91 & SS\\ 
J09044020+1725124 &   5.41 $\pm$   0.17 &   7.50 $\pm$   0.08 &   3.22 $\pm$   0.13 &   4.49 $\pm$   0.05 &   6.16 $\pm$   0.60 &   7.91 $\pm$   0.37&   8.41 $\pm$   2.05 &   6.72 $\pm$   1.79 & SS\\ 
J09072322+0948348 &   1.26 $\pm$   0.05 &   1.93 $\pm$   0.02 &   0.86 $\pm$   0.05 &   1.56 $\pm$   0.03 &   4.14 $\pm$   0.30 &   5.38 $\pm$   0.24&   7.15 $\pm$   1.89 &   4.97 $\pm$   1.20 & SS\\ 
J09142624+1024093 &   1.19 $\pm$   0.04 &   1.75 $\pm$   0.02 &   0.77 $\pm$   0.04 &   1.36 $\pm$   0.02 &   3.99 $\pm$   0.32 &   5.57 $\pm$   0.27&  10.23 $\pm$   1.91 &   6.56 $\pm$   1.25 & SS\\ 
J09193819+3336120 &   1.42 $\pm$   0.04 &   1.94 $\pm$   0.02 &   1.54 $\pm$   0.06 &   2.01 $\pm$   0.04 &   4.99 $\pm$   0.29 &   6.53 $\pm$   0.23&  14.41 $\pm$   1.68 &   9.39 $\pm$   1.08 & SS\\ 
J09354887+0937188 &   2.63 $\pm$   0.09 &   3.83 $\pm$   0.04 &   1.58 $\pm$   0.08 &   2.53 $\pm$   0.04 &   3.33 $\pm$   0.32 &   5.12 $\pm$   0.29&   5.67 $\pm$   1.91 &   4.87 $\pm$   1.38 & SS\\ 
J09381483+0200236 &   1.91 $\pm$   0.06 &   2.64 $\pm$   0.03 &   2.28 $\pm$   0.09 &   2.98 $\pm$   0.04 &   5.12 $\pm$   0.29 &   6.41 $\pm$   0.21&  17.67 $\pm$   1.78 &  10.70 $\pm$   1.06 & SS\\ 
J09405816+1904371 &   1.48 $\pm$   0.06 &   2.21 $\pm$   0.03 &   0.96 $\pm$   0.06 &   1.66 $\pm$   0.02 &   2.94 $\pm$   0.30 &   4.54 $\pm$   0.28&   3.36 $\pm$   1.76 &   3.37 $\pm$   1.35 & SS\\ 
J09473320+1005093 &  10.14 $\pm$   0.26 &  11.53 $\pm$   0.12 &  14.11 $\pm$   0.47 &  17.27 $\pm$   0.19 &  29.94 $\pm$   1.04 &  34.57 $\pm$   0.54&  64.99 $\pm$   3.18 &  80.94 $\pm$   2.26 & SS\\ 
J10005570+3140007 &   1.84 $\pm$   0.06 &   2.42 $\pm$   0.03 &   2.12 $\pm$   0.08 &   2.88 $\pm$   0.04 &   6.20 $\pm$   0.30 &   6.99 $\pm$   0.22&  14.25 $\pm$   1.91 &  15.35 $\pm$   1.31 & SS\\ 
J10222648+0911396 &   3.65 $\pm$   0.11 &   4.76 $\pm$   0.05 &   2.22 $\pm$   0.09 &   3.04 $\pm$   0.03 &   7.99 $\pm$   0.62 &   8.86 $\pm$   0.30&   6.87 $\pm$   1.63 &   6.72 $\pm$   1.40 & SS\\ 
J10335255+0044033 &   5.79 $\pm$   0.15 &   6.76 $\pm$   0.07 &   8.02 $\pm$   0.26 &   9.41 $\pm$   0.10 &  20.99 $\pm$   0.64 &  24.40 $\pm$   0.40&  69.49 $\pm$   2.96 &  69.24 $\pm$   2.12 & SS\\ 
J10340239+3452104 &  12.98 $\pm$   0.36 &  15.89 $\pm$   0.17 &   9.77 $\pm$   0.33 &  11.93 $\pm$   0.14 &  88.93 $\pm$   2.55 & 107.50 $\pm$   1.23& 223.66 $\pm$   6.06 & 216.75 $\pm$   3.37 & SS\\ 
J10375221+3125004 &   2.43 $\pm$   0.07 &   3.06 $\pm$   0.03 &   3.02 $\pm$   0.11 &   3.92 $\pm$   0.05 &   5.85 $\pm$   0.32 &   7.15 $\pm$   0.28&  12.65 $\pm$   2.01 &  13.21 $\pm$   1.41 & SS\\ 
J10500776+1132290 &   6.68 $\pm$   0.18 &   7.94 $\pm$   0.08 &   8.27 $\pm$   0.28 &  10.52 $\pm$   0.11 &  28.75 $\pm$   0.79 &  30.46 $\pm$   0.44& 110.95 $\pm$   3.73 & 105.59 $\pm$   2.46 & SS\\ 
J10500425+1205195 &   2.42 $\pm$   0.08 &   3.54 $\pm$   0.04 &   1.47 $\pm$   0.07 &   2.35 $\pm$   0.03 &   4.01 $\pm$   0.36 &   6.17 $\pm$   0.33&   5.26 $\pm$   2.16 &   4.87 $\pm$   1.68 & SS\\ 
J10523297+1036205 &   6.59 $\pm$   0.16 &   7.11 $\pm$   0.08 &  10.44 $\pm$   0.31 &  11.34 $\pm$   0.12 &  25.29 $\pm$   0.99 &  27.34 $\pm$   0.51&  85.44 $\pm$   3.04 &  94.37 $\pm$   2.34 & SS\\ 
J10542879+2049141 &   1.56 $\pm$   0.05 &   2.31 $\pm$   0.03 &   1.12 $\pm$   0.07 &   2.11 $\pm$   0.03 &   2.57 $\pm$   0.26 &   4.10 $\pm$   0.24&  10.67 $\pm$   1.53 &   7.83 $\pm$   1.14 & SS\\ 
J11052843+0736413 &   1.79 $\pm$   0.06 &   2.67 $\pm$   0.03 &   1.06 $\pm$   0.06 &   1.82 $\pm$   0.03 &   2.26 $\pm$   0.33 &   3.22 $\pm$   0.23&  -2.68 $\pm$   0.00 &   1.77 $\pm$   1.12 & SS\\ 
J11302884+1301197 &   2.14 $\pm$   0.06 &   2.82 $\pm$   0.03 &   2.52 $\pm$   0.09 &   3.25 $\pm$   0.05 &   8.98 $\pm$   0.35 &   9.61 $\pm$   0.25&  41.01 $\pm$   2.47 &  34.20 $\pm$   1.91 & SS\\ 
J11341760+1751336 &   1.19 $\pm$   0.04 &   1.94 $\pm$   0.02 &   0.72 $\pm$   0.05 &   1.36 $\pm$   0.03 &   1.80 $\pm$   0.29 &   2.81 $\pm$   0.28&  -3.75 $\pm$   0.00 &   2.19 $\pm$   1.37 & SS\\ 
J11444504+1111056 &   2.22 $\pm$   0.07 &   2.99 $\pm$   0.03 &   2.61 $\pm$   0.10 &   3.35 $\pm$   0.05 &   4.61 $\pm$   0.32 &   6.33 $\pm$   0.27&  33.06 $\pm$   2.28 &  25.32 $\pm$   1.67 & SS\\ 
J12063088+2221045 &   3.84 $\pm$   0.12 &   5.35 $\pm$   0.06 &   2.27 $\pm$   0.10 &   3.33 $\pm$   0.05 &   6.10 $\pm$   0.33 &   8.56 $\pm$   0.27&  10.49 $\pm$   1.90 &   8.70 $\pm$   1.36 & SS\\ 
J12284130+0725421 &   1.36 $\pm$   0.05 &   2.04 $\pm$   0.02 &   0.90 $\pm$   0.05 &   1.55 $\pm$   0.04 &   3.94 $\pm$   0.22 &   5.04 $\pm$   0.17&   7.66 $\pm$   1.27 &   5.17 $\pm$   0.79 & SS\\ 
J12393314+1058037 &   7.53 $\pm$   0.23 &  10.01 $\pm$   0.11 &   4.41 $\pm$   0.17 &   5.91 $\pm$   0.08 &   8.14 $\pm$   0.72 &  10.75 $\pm$   0.44&  14.17 $\pm$   2.23 &  12.37 $\pm$   2.12 & SS\\ 
J12533769+2126177 &   6.94 $\pm$   0.19 &   8.46 $\pm$   0.09 &   9.13 $\pm$   0.30 &  11.36 $\pm$   0.12 &  16.06 $\pm$   0.49 &  19.46 $\pm$   0.29&  37.48 $\pm$   1.89 &  41.68 $\pm$   1.28 & SS\\ 
J13003624+1347055 &   3.15 $\pm$   0.09 &   3.92 $\pm$   0.04 &   3.72 $\pm$   0.14 &   4.73 $\pm$   0.08 &   8.29 $\pm$   0.36 &   9.82 $\pm$   0.28&  19.97 $\pm$   2.21 &  21.02 $\pm$   1.59 & SS\\ 
J13390599+1627261 &   1.74 $\pm$   0.06 &   2.42 $\pm$   0.03 &   1.95 $\pm$   0.08 &   2.69 $\pm$   0.04 &   6.45 $\pm$   0.28 &   7.46 $\pm$   0.22&  31.41 $\pm$   2.04 &  26.12 $\pm$   1.62 & SS\\ 
J13413717+0848096 &   6.90 $\pm$   0.20 &   8.87 $\pm$   0.10 &   3.99 $\pm$   0.15 &   5.35 $\pm$   0.06 &   6.40 $\pm$   0.52 &   8.29 $\pm$   0.22&   7.20 $\pm$   1.19 &   7.30 $\pm$   1.01 & SS\\ 
J13473338+1217245 &   9.61 $\pm$   0.23 &  10.01 $\pm$   0.11 &  13.98 $\pm$   0.42 &  15.47 $\pm$   0.16 &  79.09 $\pm$   2.05 &  84.71 $\pm$   0.95& 511.20 $\pm$  10.33 & 448.47 $\pm$   5.01 & SS\\ 
J14014270+0119379 &   1.16 $\pm$   0.05 &   1.59 $\pm$   0.03 &   0.82 $\pm$   0.05 &   1.28 $\pm$   0.02 &   4.18 $\pm$   0.26 &   5.77 $\pm$   0.22&  10.03 $\pm$   1.35 &   6.94 $\pm$   0.95 & SS\\ 
J14131920+3649184 &   2.83 $\pm$   0.08 &   3.47 $\pm$   0.04 &   4.60 $\pm$   0.16 &   5.64 $\pm$   0.06 &  10.27 $\pm$   0.38 &  12.52 $\pm$   0.26&  38.25 $\pm$   1.70 &  38.63 $\pm$   1.20 & SS\\ 
J14190190+2809409 &   2.26 $\pm$   0.07 &   2.86 $\pm$   0.03 &   1.87 $\pm$   0.08 &   2.81 $\pm$   0.04 &   7.44 $\pm$   0.29 &  10.05 $\pm$   0.19&  23.89 $\pm$   1.43 &  17.45 $\pm$   1.15 & SS\\ 
J14322461+0050419 &   1.78 $\pm$   0.06 &   2.46 $\pm$   0.03 &   1.13 $\pm$   0.06 &   1.74 $\pm$   0.04 &   2.25 $\pm$   0.18 &   3.19 $\pm$   0.17&   4.16 $\pm$   1.16 &   3.85 $\pm$   0.85 & SS\\ 
J14394590+2018469 &   2.88 $\pm$   0.09 &   4.04 $\pm$   0.05 &   1.63 $\pm$   0.08 &   2.45 $\pm$   0.04 &   2.95 $\pm$   0.16 &   4.30 $\pm$   0.13&   5.68 $\pm$   0.89 &   4.58 $\pm$   0.65 & SS\\ 
J15051087+0503026 &   8.60 $\pm$   0.24 &  10.47 $\pm$   0.11 &   6.58 $\pm$   0.23 &   8.25 $\pm$   0.09 &  20.79 $\pm$   0.83 &  25.86 $\pm$   0.40&  72.33 $\pm$   2.27 &  68.06 $\pm$   1.67 & SS\\ 
J15590130+1610517 &   2.51 $\pm$   0.09 &   3.75 $\pm$   0.05 &   1.59 $\pm$   0.08 &   2.55 $\pm$   0.03 &   6.17 $\pm$   0.31 &   7.76 $\pm$   0.27&  13.75 $\pm$   1.80 &  10.62 $\pm$   1.32 & SS\\ 
J16045551+2809563 &   8.70 $\pm$   0.24 &  10.66 $\pm$   0.11 &   7.33 $\pm$   0.25 &   9.28 $\pm$   0.10 &  26.52 $\pm$   0.87 &  33.50 $\pm$   0.44&  73.61 $\pm$   2.63 &  71.70 $\pm$   2.10 & SS\\ 
J16373623+2022167 &   6.82 $\pm$   0.18 &   7.89 $\pm$   0.08 &   8.43 $\pm$   0.27 &   9.79 $\pm$   0.10 &  21.61 $\pm$   1.24 &  25.13 $\pm$   1.10&  57.03 $\pm$   2.31 &  55.83 $\pm$   1.58 & SS\\ 
J21020534-0647558 &   5.10 $\pm$   0.15 &   6.52 $\pm$   0.07 &   6.39 $\pm$   0.22 &   8.01 $\pm$   0.09 &  21.99 $\pm$   0.62 &  25.20 $\pm$   0.35&  70.18 $\pm$   2.54 &  62.35 $\pm$   1.82 & SS\\ 
J23463606+1356475 &   4.22 $\pm$   0.14 &   5.87 $\pm$   0.07 &   2.44 $\pm$   0.11 &   3.63 $\pm$   0.05 &   4.65 $\pm$   0.29 &   6.63 $\pm$   0.25&   7.18 $\pm$   1.63 &   5.78 $\pm$   1.20 & SS\\ 
IC2218 &   7.85 $\pm$   0.20 &   9.10 $\pm$   0.10 &   4.26 $\pm$   0.14 &   5.00 $\pm$   0.05 &   3.81 $\pm$   0.44 &   5.42 $\pm$   0.27&  -3.29 $\pm$   0.00 &   2.55 $\pm$   1.31 & HI\\ 
NGC2620 &  25.28 $\pm$   0.62 &  27.75 $\pm$   0.29 &  13.92 $\pm$   0.42 &  15.83 $\pm$   0.17 &  17.87 $\pm$   1.11 &  22.12 $\pm$   0.73&  21.57 $\pm$   3.19 &  22.90 $\pm$   3.39 & HI\\ 
NGC2713 & 165.41 $\pm$   3.92 & 174.96 $\pm$   1.84 &  88.82 $\pm$   2.55 &  95.88 $\pm$   1.01 &  93.72 $\pm$   3.54 & 125.54 $\pm$   1.76& 109.59 $\pm$   6.49 & 124.50 $\pm$   6.11 & HI\\ 
IC2446 &  31.11 $\pm$   0.77 &  34.35 $\pm$   0.36 &  17.29 $\pm$   0.52 &  19.23 $\pm$   0.20 &  33.19 $\pm$   1.80 &  32.92 $\pm$   0.47&  35.25 $\pm$   1.91 &  37.45 $\pm$   1.60 & HI\\ 
IC536 &  20.05 $\pm$   0.50 &  22.27 $\pm$   0.23 &  10.76 $\pm$   0.33 &  12.15 $\pm$   0.13 &   9.29 $\pm$   0.76 &  12.34 $\pm$   0.48&   4.84 $\pm$   2.39 &   6.73 $\pm$   2.32 & HI\\ 
UGC05830 &  16.18 $\pm$   0.43 &  19.06 $\pm$   0.20 &   9.36 $\pm$   0.30 &  10.92 $\pm$   0.12 &  26.56 $\pm$   1.14 &  31.51 $\pm$   0.52&  38.04 $\pm$   2.86 &  36.94 $\pm$   2.05 & HI\\ 
UGC06066 &  12.27 $\pm$   0.32 &  14.12 $\pm$   0.15 &   6.35 $\pm$   0.20 &   7.51 $\pm$   0.08 &   3.01 $\pm$   0.53 &   5.26 $\pm$   0.41&   3.86 $\pm$   2.14 &   4.71 $\pm$   2.02 & HI\\ 
UGC08179 &  17.80 $\pm$   0.47 &  20.77 $\pm$   0.22 &  10.76 $\pm$   0.36 &  12.89 $\pm$   0.15 &  44.66 $\pm$   1.51 &  53.20 $\pm$   0.68&  89.02 $\pm$   5.15 &  79.70 $\pm$   2.18 & HI\\ 
IC881 &  22.58 $\pm$   0.57 &  25.27 $\pm$   0.27 &  11.78 $\pm$   0.37 &  13.35 $\pm$   0.15 &   0.37 $\pm$   0.19 &   4.32 $\pm$   0.16&   1.20 $\pm$   1.04 &   2.20 $\pm$   0.82 & HI\\ 
UGC08902 &  36.86 $\pm$   0.88 &  39.25 $\pm$   0.42 &  21.47 $\pm$   0.63 &  23.24 $\pm$   0.26 &  60.75 $\pm$   1.93 &  69.08 $\pm$   0.84& 113.50 $\pm$   4.44 & 113.13 $\pm$   2.40 & HI\\ 
NGC5417 &  56.89 $\pm$   1.39 &  62.05 $\pm$   0.65 &  29.99 $\pm$   0.89 &  32.93 $\pm$   0.35 &  15.50 $\pm$   0.99 &  25.93 $\pm$   0.58&  21.27 $\pm$   2.58 &  25.08 $\pm$   2.61 & HI\\ 
NGC5440 &  98.16 $\pm$   2.35 & 105.05 $\pm$   1.10 &  50.48 $\pm$   1.46 &  53.53 $\pm$   0.56 &  29.82 $\pm$   2.33 &  45.00 $\pm$   0.81&  41.04 $\pm$   4.85 &  47.21 $\pm$   3.52 & HI\\ 
UGC09195 &   9.04 $\pm$   0.25 &  11.15 $\pm$   0.12 &   5.01 $\pm$   0.17 &   6.33 $\pm$   0.07 &   8.32 $\pm$   0.49 &  10.95 $\pm$   0.31&  12.94 $\pm$   1.60 &  12.43 $\pm$   1.49 & HI\\ 
NGC5635 &  85.45 $\pm$   2.07 &  92.28 $\pm$   0.97 &  45.24 $\pm$   1.32 &  49.14 $\pm$   0.53 &  31.80 $\pm$   1.72 &  46.95 $\pm$   0.73&  41.39 $\pm$   3.48 &  48.20 $\pm$   2.85 & HI\\ 
NGC5790 &  20.22 $\pm$   0.53 &  23.18 $\pm$   0.25 &  11.23 $\pm$   0.37 &  13.40 $\pm$   0.16 &  13.42 $\pm$   0.68 &  18.97 $\pm$   0.48&  21.07 $\pm$   2.11 &  23.17 $\pm$   2.17 & HI\\ 
UGC09757 &  17.67 $\pm$   0.45 &  19.95 $\pm$   0.21 &  10.21 $\pm$   0.32 &  11.88 $\pm$   0.14 &  27.36 $\pm$   0.95 &  32.83 $\pm$   0.49&  36.58 $\pm$   2.00 &  38.52 $\pm$   1.76 & HI\\ 
UGC09795 &  12.09 $\pm$   0.31 &  14.03 $\pm$   0.15 &   7.19 $\pm$   0.23 &   8.37 $\pm$   0.09 &  20.56 $\pm$   0.99 &  23.73 $\pm$   0.38&  23.43 $\pm$   1.77 &  23.73 $\pm$   1.42 & HI\\ 
UGC12591 & 105.43 $\pm$   2.63 & 117.27 $\pm$   1.23 &  54.37 $\pm$   1.67 &  60.20 $\pm$   0.64 &  18.14 $\pm$   1.35 &  37.63 $\pm$   1.08&  21.17 $\pm$   4.46 &  31.21 $\pm$   5.21 & HI\\ 


==> Table5.tex <==
2MFGC12344 &   58.0 $\pm$    1.4 &   0.99  &  11.65 \\ 
OGC~139 &   38.2 $\pm$    0.9 &   1.14  &  11.65 \\ 
OGC~217 &   66.7 $\pm$    4.6 &   1.89  &  11.56 \\ 
OGC~290 &   64.2 $\pm$    1.8 &   1.78  &  11.65 \\ 
OGC~345 &   59.6 $\pm$    2.3 &   1.19  &  11.61 \\ 
OGC~454 &   52.8 $\pm$    4.4 &   1.49  &  11.54 \\ 
OGC~543 &  326.8 $\pm$    6.9 &   1.17  &  11.53 \\ 
OGC~586 &   55.1 $\pm$    2.7 &   1.28  &  11.54 \\ 
OGC~595 &   53.9 $\pm$    1.4 &   1.12  &  11.43 \\ 
OGC~789 &  149.4 $\pm$    3.4 &   1.21  &  11.51 \\ 
OGC~800 &  133.8 $\pm$    3.9 &   1.01  &  11.53 \\ 
OGC~830 &   55.1 $\pm$    4.1 &   1.06  &  11.56 \\ 
OGC~926 &  109.4 $\pm$    2.5 &   1.47  &  11.56 \\ 
OGC~928 &   45.0 $\pm$    2.8 &   1.26  &  11.56 \\ 
OGC~968 &   86.6 $\pm$    2.2 &   1.81  &  11.51 \\ 
OGC~1250 &   78.6 $\pm$    2.0 &   0.94  &  11.38 \\ 
OGC~1273 &   42.2 $\pm$    2.5 &   1.04  &  11.42 \\ 
OGC~1304 &  388.8 $\pm$   11.9 &   1.44  &  11.53 \\ 
OGC~1379 & --  &   1.11  &  11.45 \\ 
OGC~1457 & --  &   1.41  &  11.39 \\ 
OGC~1464 &   22.2 $\pm$    2.3 &   1.54  &  11.54 \\ 
OGC~1546 &   59.0 $\pm$    4.1 &   0.72  &  11.50 \\ 
OGC~1559 &  248.7 $\pm$    5.4 &   0.94  &  11.56 \\ 
J01593759+1231120 &  108.9 $\pm$    4.8 &   1.35  &  11.46 \\ 
J08185186+1013117 &  103.0 $\pm$    4.1 &   0.63  &  11.28 \\ 
J09044020+1725124 &  110.6 $\pm$    4.8 &   0.81  &  11.49 \\ 
J09072322+0948348 & --  &   1.29  &  11.48 \\ 
J09142624+1024093 &   11.0 $\pm$    0.4 &   1.38  &  11.44 \\ 
J09354887+0937188 &   45.7 $\pm$    3.2 &   0.83  &  11.52 \\ 
J09405816+1904371 &    6.9 $\pm$    0.2 &   0.86  &  11.44 \\ 
J10222648+0911396 &  118.5 $\pm$    2.6 &   0.73  &  11.31 \\ 
J10340239+3452104 & --  &   1.70  &  11.63 \\ 
J10500425+1205195 &  102.8 $\pm$    2.1 &   0.99  &  11.50 \\ 
J10542879+2049141 &   53.5 $\pm$    3.0 &   1.51  &  11.63 \\ 
J11052843+0736413 & --  &   0.92  &  11.48 \\ 
J11341760+1751336 & --  &   0.97  &  11.46 \\ 
J12063088+2221045 &  154.9 $\pm$    7.8 &   1.04  &  11.47 \\ 
J12284130+0725421 &   35.6 $\pm$    0.9 &   1.21  &  11.42 \\ 
J12393314+1058037 &  118.8 $\pm$    2.8 &   0.79  &  11.44 \\ 
J13413717+0848096 &   44.8 $\pm$    3.4 &   0.53  &  11.45 \\ 
J14014270+0119379 & --  &   1.07  &  11.20 \\ 
J14322461+0050419 &   10.5 $\pm$    0.3 &   0.67  &  11.28 \\ 
J14394590+2018469 &   35.9 $\pm$    3.2 &   0.81  &  11.45 \\ 
J15051087+0503026 &  149.1 $\pm$    3.4 &   1.42  &  11.48 \\ 
J15590130+1610517 &  108.1 $\pm$    4.4 &   1.34  &  11.54 \\ 
J23463606+1356475 &   31.5 $\pm$    0.7 &   0.87  &  11.60 \\ 
IC2218 & --  &   0.09  &  10.96 \\ 
NGC2620 &  512.3 $\pm$   10.5 &   0.15  &  11.02 \\ 
NGC2713 & 1639.6 $\pm$   33.1 &   0.18  &  11.23 \\ 
IC2446 &  359.3 $\pm$    9.5 &   0.27  &  11.12 \\ 
IC536 &  142.5 $\pm$    3.9 &  -0.16  &  10.96 \\ 
UGC05830 & --  &   0.85  &  11.29 \\ 
UGC06066 &  231.1 $\pm$    4.8 &  -0.03  &  11.07 \\ 
UGC08179 &  762.7 $\pm$   19.0 &   1.25  &  11.48 \\ 
IC881 &  126.1 $\pm$    3.4 & $<$  -0.89  &  10.87 \\ 
UGC08902 & 1660.8 $\pm$   37.4 &   0.78  &  11.17 \\ 
NGC5417 &  475.4 $\pm$   12.5 &  -0.28  &  10.96 \\ 
NGC5440 &  610.3 $\pm$   21.2 &  -0.30  &  10.95 \\ 
UGC09195 &  440.4 $\pm$   12.5 &   0.57  &  11.15 \\ 
NGC5635 & 1266.1 $\pm$   35.6 &  -0.05  &  11.03 \\ 
NGC5790 &  418.0 $\pm$   12.4 &   0.42  &  11.23 \\ 
UGC09757 &  750.1 $\pm$   15.7 &   0.74  &  11.25 \\ 
UGC09795 &  227.0 $\pm$    7.5 &   0.55  &  11.17 \\ 
UGC12591 &  210.4 $\pm$    5.9 &  -0.06  &  11.54 \\ 

